Remarks on Category-Based Routing in Social Networks

It is well known that individuals can route messages on short paths through social networks, given only simple information about the target and using only local knowledge about the topology. Sociologists conjecture that people find routes greedily by passing the message to an acquaintance that has more in common with the target than themselves, e.g. if a dentist in Saarbr\"ucken wants to send a message to a specific lawyer in Munich, he may forward it to someone who is a lawyer and/or lives in Munich. Modelling this setting, Eppstein et al. introduced the notion of category-based routing. The goal is to assign a set of categories to each node of a graph such that greedy routing is possible. By proving bounds on the number of categories a node has to be in we can argue about the plausibility of the underlying sociological model. In this paper we substantially improve the upper bounds introduced by Eppstein et al. and prove new lower bounds.

==> bookmacros.tex <==

\newcommand{\semph}[1]{\mbox{}{\color{blue} #1}}


\newcommand{\widebinop}[1]{\hspace{0.5em}#1\hspace{0.5em}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}


\newcommand{\donotshow}[1]{}
\newcommand{\maths}{mathematics'}
\newcommand{\apostrophe}{'}
\newcommand{\dapostrophe}{''}

\newcommand{\ignore}[1]{}
\newcommand{\pnegskip}{\vspace*{-\baselineskip}\vspace*{-\belowdisplayskip}\par}

\newcommand{\proofendswithequation}{\vspace*{-\baselineskip}\vspace*{-\belowdisplayskip}\par}

\newcommand{\eqndot}{\ .}\newcommand{\eqncomma}{\ ,}

\newcommand{\tildeO}{\widetilde{O}}
\newcommand{\Otilde}{\tildeO}



\providecommand{\mod}{\mathop{\rm mod}}
\newcommand{\conv}{\mathop{\rm conv}}

\newcommand{\F}{{\cal F}}

\newcommand{\dom}{\mathop{\rm dom}\nolimits}
\newcommand{\op}{\mathbin{\rm op}}
\newcommand{\mes}{\mathop {\rm mes}}
\newcommand{\ind}{\mathop {\rm ind}}
\newcommand{\size}{\mathop {\rm size}}
\newcommand{\fl}{\mathop {\rm fl}}

\newcommand{\cl}{\mathop {\rm cl}}
\newcommand{\inn}{\mathop {\rm int}}
\newcommand{\cpl}{\mathop {\rm cpl}}
\newcommand{\reg}{\mathop {\rm reg}}
\newcommand{\bd}{\mathop {\rm bd}}
\newcommand{\bR}{\mathop {\rm bR}}



%\newcommand{\cp}{\mbox{$\:cp$}}
%\newcommand{\mac}{\mbox{$\:mac$}}
%\newcommand{\cmp}{\mbox{$\:cmp$}}
%\newcommand{\ops}{\mbox{$\:ops$}}

\newcommand{\loglog}{\mathop {\rm loglog}}
\newcommand{\lnln}{\mathop {\rm lnln}}
\newcommand{\assign}{\mathbin{\raisebox{0.05ex}{\mbox{\rm :}}\!\!=}}
\newcommand{\define}{\mathbin{\raisebox{0.05ex}{\mbox{\rm :}}\!\!=}}


\newcommand{\CC}{C\raisebox{.08ex}{\hbox{\tt ++}}}
\newcommand{\Cminus}{C\raisebox{.08ex}{\hbox{\tt ++}}\raisebox{.25ex}{-}}
\newcommand{\GG}{g\raisebox{.08ex}{\hbox{\tt ++}}}
\newcommand{\Gminus} {g\raisebox{.08ex}{\hbox{\tt ++}}\raisebox{.25ex}{-}}
%\newcommand{\R}{I\! \!R}
%\newcommand{\N}{I\! \!N}
%\newcommand{\Z}{I\! \!Z}
%\providecommand{\R}{\mathbb{R}}
\newcommand{\RR}{\mathbb{R}}
\providecommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Rp}{\mathbb{R}_{>0}}
\newcommand{\Rn}{\mathbb{R}_{<0}}
\newcommand{\Rnn}{\mathbb{R}_{\ge 0}}
\newcommand{\Nnull}{\mathbb{N}_{0}}

\newcommand{\Oh}[1]{{\rm O}(#1)}
\newcommand{\OhL}[1]{{\rm O}\left(#1\right)}


\newcommand{\progitem}[1]{$\langle$#1$\rangle$ }
\newcommand {\abs}[1] {| #1 |}


\renewcommand{\topfraction}{1}
\renewcommand{\textfraction}{0}
\renewcommand{\bottomfraction}{0.5}


\newenvironment{remark}{{\bf Remark:}}{\par}

\newcommand{\strecke}[2]{{#1#2}$^{\hspace{-.6cm}\longrightarrow}$ \ }
\newcommand{\punktstrecke}[2]{{#1#2}$^{\hspace{-.6cm}\longrightarrow}\ $}



%Basicdatatypes/papermacros.tex

\providecommand{\3}{\ss}
%\newcommand{\ck}{\discretionary{k-}{k}{ck}}



%\newcommand{\abs}[1]{| #1 |}

\newcommand{\la}{$\langle$}
\newcommand{\ra}{$\rangle$\ }
%\newcommand{\Litem}[2]{$\langle$#1,#2$\rangle$\ }
\newcommand{\Listitem}[1]{$\langle$#1$\rangle$\ }

%\newcommand{\range}[2]{[#1 \, \ldots \, #2]}
\providecommand{\range}[2]{[#1\, ..\,  #2]}

%\newcommand{\halfrange}[2]{[#1 \, \ldots \, #2)}
\newcommand{\halfrange}[2]{[#1\,  ..\,  #2)}


%\newcommand{\precond}{\\ {\em precondition}: }

\newcommand{\Msection}[1]{\\
\medskip 
{ \large {\bf #1}}\\  
\smallskip

}

\newcommand{\Msubsection}[1]{\\
\medskip
{\bf #1}\\ 
\smallskip

}


\newcommand{\Kurt}{\htmladdnormallink{Kurt Mehlhorn}{http://www.mpi-sb.mpg.de/\~{}mehlhorn}}
\newcommand{\Stefan}{\htmladdnormallink{Stefan N\"aher}{http://www.informatik.uni-halle.de/\~{}naeher}}
\newcommand{\Christian}{\htmladdnormallink{Christian Uhrig}{http://www.mpi-sb.mpg.de/\~{}uhrig}}
\newcommand{\LEDA}{\htmladdnormallink{LEDA}{http://www.mpi-sb.mpg.de/LEDA/leda.html}}
\newcommand{\GmbH}{\htmladdnormallink{LEDA Software
GmbH}{http://www.mpi-sb.mpg.de/LEDA/GMBH/gmbh.html}}

\newcommand{\SB}{Saarbr\"{u}cken}

\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{\ref{fig:#1}}
\newcommand{\Hline}{\hspace{0.0in}\hrulefill\hspace{0.0in}}


\newcommand{\Figger}[3]{
    \begin{figure}[thbp]
      \Hline
      \begin{center}
      \input{figs/#3}
      \end{center}
      \caption{#2}\figlabel{#1}
      \Hline
    \end{figure}
    }

\newcommand{\topFigger}[3]{
    \begin{figure}[t]
      \Hline
      \begin{center}
      \input{figs/#3}
      \end{center}
      \caption{#2}\figlabel{#1}
      \Hline
    \end{figure}
    }

\newcommand{\bottomFigger}[3]{
    \begin{figure}[b]
      \Hline
      \begin{center}
      \input{figs/#3}
      \end{center}
      \caption{#2}\figlabel{#1}
      \Hline
    \end{figure}
    }

\newcommand{\topbottomFigger}[3]{
    \begin{figure}[tb]
      \Hline
      \begin{center}
      \input{figs/#3}
      \end{center}
      \caption{#2}\figlabel{#1}
      \Hline
    \end{figure}
    }

\newcommand{\hereFigger}[3]{
    \begin{figure}[h]
      \Hline
      \begin{center}
      \input{figs/#3}
      \end{center}
      \caption{#2}\figlabel{#1}
      \Hline
    \end{figure}
    }

\newcommand{\allFigger}[3]{
    \begin{figure}[htbp]
      \Hline
      \begin{center}
      \input{figs/#3}
      \end{center}
      \caption{#2}\figlabel{#1}
      \Hline
    \end{figure}
    }



\newlength{\setspacing}
\setlength{\setspacing}{0.05em}

%\providecommand{\sset}[1]{\{\, #1 \,\}}
\providecommand{\sset}[1]{\{\, #1 \,\}}
%\newcommand{\set}[2]{ \left\{\, #1 \mbox{ ; } #2 \,\right\}  }
\providecommand{\set}[2]{ \left\{\, #1 \mbox{{\rm ; }} #2 \, \right\}  }

\newcommand{\uedge}[1]{\sset{#1}}

%\providecommand{\path}[1]{[\hspace{\setspacing} #1 \hspace{\setspacing}]}
\providecommand{\Path}[1]{[\hspace{\setspacing} #1 \hspace{\setspacing}]}
\newcommand{\seq}[1]{(\hspace{\setspacing} #1 \hspace{\setspacing} )}

\newcommand{\Exp}[1]{{\rm E}[ #1 ]}
\newcommand{\Cexp}[2]{{\rm E}[ #1 \,|\, #2]}
\newcommand{\prob}[1]{{\rm prob}( #1 )}
\newcommand{\cprob}[2]{{\rm prob}(#1 \,|\, #2)}


\newcommand{\disjointcup}{\mathbin {\dot{\cup}}}

\newcommand{\Kmarginpar}[1]{\marginpar{\footnotesize #1}}






\newcommand{\mbegin}{\{\ \ }
\newcommand{\mend}{\}}
\newcommand{\memptyline}{\\[-2ex]}

\newlength{\mleftindent}
\setlength{\mleftindent}{\parindent}
\newlength{\mindent}
\settowidth{\mindent}{\mbegin}
\newlength{\mboxwidth}
\newcommand{\mincrement}{\addtolength{\mboxwidth}{-\mindent}}
\newcommand{\mdecrement}{\addtolength{\mboxwidth}{\mindent}}



\newlength{\preprogramskip}
\newlength{\postprogramskip}
\setlength{\preprogramskip}{\smallskipamount}
\setlength{\postprogramskip}{\smallskipamount}

\newcommand{\mprogram}[1]
{\vspace{\preprogramskip}
 \setlength{\mboxwidth}{\linewidth}%
 \addtolength{\mboxwidth}{-\parindent}\par
 \parbox[t]{\mboxwidth}{#1}
 \vspace{\postprogramskip}\par%
}



\newlength{\mexpwidth}
\newlength{\mexpindent}
\newcommand{\indentafterkeyword}{\hspace*{0.5em}}




\newcommand{\mcommand}[3]
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf #1\indentafterkeyword}}%
\addtolength{\mexpwidth}{-\mexpindent}%
{\bf #1\indentafterkeyword}\parbox[t]{\mexpwidth}{#2}\\
\mincrement
\mbegin \parbox[t]{\mboxwidth}{#3}\\
\mend
\mdecrement
}

\newcommand{\mscommand}[3]
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf #1\indentafterkeyword}}%
\addtolength{\mexpwidth}{-\mexpindent}%
{\bf #1\indentafterkeyword}\parbox[t]{\mexpwidth}{#2}\\
\mincrement
\mbegin \parbox[t]{\mboxwidth}{#3 \mend}
\mdecrement
}

\newcommand{\monelinecommand}[3]
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf #1\indentafterkeyword}}%
\addtolength{\mexpwidth}{-\mexpindent}%
{\bf #1\indentafterkeyword}{#2}%
\mbegin #3 \mend
}


\newcommand{\mwhile}[2]
{\mcommand{while}{#1}{#2}}

\newcommand{\mforall}[2]
{\mcommand{forall}{#1}{#2}}

\newcommand{\monelineforall}[2]
{\monelinecommand{forall}{#1}{#2}}

\newcommand{\mforalledges}[2]
{\mcommand{forall\_edges}{#1}{#2}}

\newcommand{\mifthen}[2]
{\mcommand{if}{#1}{#2}}


\newcommand{\mswhile}[2]
{\mscommand{while}{#1}{#2}}

\newcommand{\monelinewhile}[2]
{\monelinecommand{while}{#1}{#2}}

\newcommand{\msforall}[2]
{\mscommand{forall}{#1}{#2}}

\newcommand{\msforalledges}[2]
{\mscommand{forall\_edges}{#1}{#2}}

\newcommand{\msifthen}[2]
{\mscommand{if}{#1}{#2}}

\newcommand{\monelineifthen}[2]
{{\bf if} #1  #2}

\newcommand{\monelineif}[2]
{{\bf if} #1  #2}





\newcommand{\mifelse}[3]
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf if\indentafterkeyword}}%
\addtolength{\mexpwidth}{-\mexpindent}%
{\bf if\indentafterkeyword}\parbox[t]{\mexpwidth}{#1}\\
\mincrement \mbegin \parbox[t]{\mboxwidth}{#2}\\
\mend \mdecrement \\
{\bf else} \\
\mincrement \mbegin \parbox[t]{\mboxwidth}{#3}\\
\mend \mdecrement
}

\newcommand{\mslifelse}[3]  %if is short else is long
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf if\indentafterkeyword}}%
\addtolength{\mexpwidth}{-\mexpindent}%
{\bf if\indentafterkeyword}\parbox[t]{\mexpwidth}{#1}\\
\mincrement \mbegin \parbox[t]{\mboxwidth}{#2 \mend} \mdecrement \\
{\bf else} \\
\mincrement \mbegin \parbox[t]{\mboxwidth}{#3}\\
\mend \mdecrement
}

\newcommand{\mlsifelse}[3]
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf if\indentafterkeyword}}%
\addtolength{\mexpwidth}{-\mexpindent}%
{\bf if\indentafterkeyword}\parbox[t]{\mexpwidth}{#1}\\
\mincrement \mbegin \parbox[t]{\mboxwidth}{#2}\\
\mend \mdecrement \\
{\bf else} \\
\mincrement \mbegin \parbox[t]{\mboxwidth}{#3 \mend} \mdecrement
}

\newcommand{\mssifelse}[3]
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf if\indentafterkeyword}}%
\addtolength{\mexpwidth}{-\mexpindent}%
{\bf if\indentafterkeyword}\parbox[t]{\mexpwidth}{#1}\\
\mincrement \mbegin \parbox[t]{\mboxwidth}{#2 \mend} \mdecrement \\
{\bf else} \\
\mincrement \mbegin \parbox[t]{\mboxwidth}{#3 \mend} \mdecrement
}

\newcommand{\mtwolineifelse}[3]
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf if\indentafterkeyword}}%
\addtolength{\mexpwidth}{-\mexpindent}%
{\bf if\indentafterkeyword}#1 \mbegin #2 \mend \\
{\bf else} \mbegin #3 \mend % 
}

\newcommand{\monelineifelse}[3]
{ {\bf if} #1 \mbegin #2 \mend \ \ {\bf else}\ \ \mbegin #3 \mend }




\newcommand{\mbreak}{{\bf break}}
\newcommand{\mcomment}[1]{/* #1 */}

\newcommand{\mdo}[2]
{\mcommand{do}{#1}{#2}}

\newcommand{\msdo}[2]
{\mscommand{do}{#1}{#2}}

\providecommand{\Path}[1]{[#1]}


\newenvironment{citemize}% compressed itemize with small preskip
{\vspace{-0.3em}\begin{itemize}
\setlength{\itemsep}{0.2\itemsep}%
\setlength{\parskip}{0.2\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
\setlength{\topsep}{0.0\topsep}%
%\renewcommand{\makelabel}{\citem}
}
{\end{itemize}}

\newenvironment{ccitemize}% compressed itemize with standard preskip
{\begin{itemize}
\setlength{\itemsep}{0.2\itemsep}%
\setlength{\parskip}{0.2\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
\setlength{\topsep}{0.0\topsep}%
%\renewcommand{\makelabel}{\citem}
}
{\end{itemize}}

\newenvironment{eitemize}% expanded itemize with standard preskip
{\begin{itemize}
\setlength{\itemsep}{1.5\itemsep}%
\setlength{\parskip}{1.5\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
\setlength{\topsep}{0.0\topsep}%
%\renewcommand{\makelabel}{\citem}
}
{\end{itemize}}

\newenvironment{eeitemize}% expanded itemize with expanded preskip
{\begin{itemize}
\setlength{\itemsep}{1.5\itemsep}%
\setlength{\parskip}{1.5\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
%\setlength{\topsep}{10.0\topsep}%
%\renewcommand{\makelabel}{\citem}
\par \smallskip
}
{\end{itemize}}

\newenvironment{eeeitemize}% expanded itemize with expanded preskip
{\begin{itemize}
\setlength{\itemsep}{1.5\itemsep}%
\setlength{\parskip}{1.5\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
%\setlength{\topsep}{10.0\topsep}%
%\renewcommand{\makelabel}{\citem}
\par \medskip
}
{\end{itemize}}

\newenvironment{cdescription}% compressed description with small preskip
{\vspace{-0.3em}\begin{description}
\setlength{\itemsep}{0.2\itemsep}%
\setlength{\parskip}{0.2\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
\setlength{\topsep}{0.0\topsep}%
%\renewcommand{\makelabel}{\citem}
}
{\end{description}}

\newenvironment{ccdescription}% compressed description with standard preskip
{\begin{description}
\setlength{\itemsep}{0.2\itemsep}%
\setlength{\parskip}{0.2\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
\setlength{\topsep}{0.0\topsep}%
%\renewcommand{\makelabel}{\citem}
}
{\end{description}}

\newenvironment{cenumerate}% compressed itemize with small preskip
{\vspace{-0.3em}\begin{enumerate}
\setlength{\itemsep}{0.2\itemsep}%
\setlength{\parskip}{0.2\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
\setlength{\topsep}{0.0\topsep}%
%\renewcommand{\makelabel}{\citem}
}
{\end{enumerate}}

\newenvironment{ccenumerate}% compressed itemize with standard preskip
{\begin{enumerate}
\setlength{\itemsep}{0.2\itemsep}%
\setlength{\parskip}{0.2\parskip}%
%\setlength{\labelwidth}{350pt}%
%\setlength{\leftmargin}{\labelwidth+\labelsep}%
\setlength{\topsep}{0.0\topsep}%
%\renewcommand{\makelabel}{\citem}
}
{\end{enumerate}}


\newcommand{\mindentcommand}[3]
{\setlength{\mexpwidth}{\mboxwidth}%
\settowidth{\mexpindent}{{\bf #1}\indentafterkeyword #2}%
\addtolength{\mboxwidth}{-\mexpindent}%
{\bf #1}\indentafterkeyword #2 \mbegin%
\parbox[t]{\mboxwidth}{#3}\\%
\hspace*{\mexpindent}\mend%
\addtolength{\mboxwidth}{\mexpindent}
}







==> papermacros.tex <==
\input bookmacros.tex

\newlength{\proofpostskipamount}\newlength{\proofpreskipamount}
\setlength{\proofpreskipamount}{0.1ex}

\setlength{\proofpostskipamount}{0.1ex}


\newenvironment{proof}%
               {\par\vspace{\proofpreskipamount}\noindent{\bf Proof:}\hspace{0.5em}}% 0.5 before
               {\nopagebreak%
                \strut\nopagebreak%
                \hspace{\fill}\qed\par\vspace{\proofpostskipamount}\noindent}

\newenvironment{Proof}[1]%
               {\par\vspace{0.5ex}\noindent{\bf Proof #1:}\hspace{0.5em}}%
               {\nopagebreak%
                \strut\nopagebreak%
                \hspace{\fill}\qed\par\medskip\noindent}


\newcommand{\highqed}{\vspace{-\belowdisplayskip -2.0\baselineskip}\par}


\newenvironment{exercises}
{\paragraph{Exercises:}\nopagebreak[5]
\begin{enumerate}
}
{\end{enumerate}}


\newtheorem{exercise}{Exercise}

\newcommand{\acsthanks}{\thanks{
Partially supported by the IST Programme of the EU as a Shared-corst RTD
(FET
Open) Project under Contract No IST-006413 (ACS - Algorithms for Complex
Shapes)}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{task}{Task}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}
\providecommand{\qed}{\rule[-0.2ex]{0.3em}{1.4ex}}


\newtheorem{Laxiom}{LEDA Axiom}
\newtheorem{Caxiom}{\CC\ Axiom}
\newtheorem{Lrule}{LEDA Rule}
\newtheorem{fact}{Fact}
\newtheorem{claim}{Claim}


\newlength{\mydefwidth}
\newlength{\mytextwidth}

\newcommand{\slidedef}[3]{
        \settowidth{\mydefwidth}{#2}%
  \setlength{\mytextwidth}{\textwidth}%
        \addtolength{\mytextwidth}{-#1}%
        \noindent\parbox[t]{#1}{#2}%     
        \parbox[t]{\mytextwidth}{\sloppy #3}%
         }

\newtheorem{question}{Question}
%\newtheorem{definition}{Definition}

\newcommand{\myurl}[1]{{\footnotesize \url{#1}}}
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathllapinternal#1#2{%
\llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{%
\rlap{$\mathsurround=0pt#1{#2}$}}
\def\mathclapinternal#1#2{%
\clap{$\mathsurround=0pt#1{#2}$}}




